Bandits and Experts in Metric Spaces

In a multi-armed bandit problem, an online algorithm chooses from a set of strategies in a sequence of trials so as to maximize the total payoff of the chosen strategies. While the performance of bandit algorithms with a small finite strategy set is quite well understood, bandit problems with large strategy sets are still a topic of very active investigation, motivated by practical applications such as online auctions and web advertisement. The goal of such research is to identify broad and natural classes of strategy sets and payoff functions which enable the design of efficient solutions. In this work we study a very general setting for the multi-armed bandit problem in which the strategies form a metric space, and the payoff function satisfies a Lipschitz condition with respect to the metric. We refer to this problem as the "Lipschitz MAB problem". We present a solution for the multi-armed bandit problem in this setting. That is, for every metric space we define an isometry invariant which bounds from below the performance of Lipschitz MAB algorithms for this metric space, and we present an algorithm which comes arbitrarily close to meeting this bound. Furthermore, our technique gives even better results for benign payoff functions. We also address the full-feedback ("best expert") version of the problem, where after every round the payoffs from all arms are revealed.

==> sec-experts-overview.tex <==
\section{The \FFproblem [DEPRECATED!]}
\label{sec:experts-overview}

We turn our attention to the \emph{\FFproblem}: the full-feedback version of the \problem. This section defines the problem and overviews our contributions for this problem. Proofs of the theorems stated in this section will be deferred to the following three sections.

\xhdr{Problem definition.}
A problem instance is specified by a triple $(X,\mD,\prob)$, where $(X,\mD)$ is a metric space and $\prob$ is a  probability measure with universe $[0,1]^X$, the set of all functions from $X$ to $[0,1]$, such that the expected payoff function
    $\mu: x \mapsto \E_{f \in \prob}[f(x)]$
is a Lipschitz function on $(X,\mD)$. The metric structure of $(X,\mD)$ is known to the algorithm, the measure $\prob$ is not. We will refer to $\prob$ as the problem instance when the metric space $(X,\mD)$ is clear from the context.

In each round $t$ the algorithm picks a strategy $x_t\in X$, then
the environment chooses an independent sample $f_t: X\to [0,1]$ distributed according to the measure $\prob$. The algorithm receives payoff $f_t(x_t)$, and also observes the entire payoff function $f_t$. More formally, the algorithm can query the value of $f_t$ at an arbitrary finite number of points. Some of our upper bounds are for a (very) restricted version, called \emph{double feedback}, where in each round the algorithm picks two arms $(x,y)$, receives the payoff for $x$ and also observes the payoff for $y$. By abuse of notation, we will treat the bandit setting as a special case of the experts setting.

Note that the payoffs for different arms in a given round are not necessarily independent. This is essential because for any limit point $x$ in the metric space one could use many independent samples from the vicinity of $x$ to learn the expected payoff at $x$ in a single round.

\xhdr{Regret dichotomies.}
We show that the \FFproblem exhibits a regret dichotomy similar to the one in Theorem~\ref{thm:intro-dichotomy-MAB}. It is known that the optimal regret for a finite strategy set is \emph{constant} \citep{sleeping-colt08}. Accordingly, the dichotomy is between $O(1)$ and $\sqrt{t}$ regret.

\begin{theorem}\label{thm:main-experts}
The \FFproblem on metric space $(X,\mD)$ is either $1$-tractable, even with double feedback, or it is not $g(t)$-tractable for any $g\in o(\sqrt{t})$, even with full feedback. The former occurs if and only if the completion of $X$ is a compact metric space with countably many points.
\end{theorem}

Theorem~\ref{thm:main-experts} and its bandit counterpart (Theorem~\ref{thm:intro-dichotomy-MAB}) are proved jointly in Section~\ref{sec:dichotomies}, using essentially the same ideas. In both theorems, the regret dichotomy corresponds to the transition form countable to uncountable strategy set (assuming the metric space is compact and complete). Note that the upper bound in Theorem~\ref{thm:main-experts} only assumes double feedback, whereas the lower bound is for the unrestricted full feedback.



Next, we investigate for which metric spaces the \FFproblem is $o(t)$-tractable. We extend Theorem~\ref{thm:boundary-of-tractability-bandits} for the \problem to another regret dichotomy where the upper bound is for the bandit setting, whereas the lower bound is for full feedback. We prove this result in Section~\ref{sec:boundary-body}.

\begin{theorem}\label{thm:boundary-of-tractability}
The \FFproblem on metric space $(X,\mD)$ is either $f(t)$-tractable for some $f\in o(t)$, even in the bandit setting, or it is not $g(t)$-tractable for any $g\in o(t)$, even with full feedback. The former occurs if and only if the completion of $X$ is a compact metric space.
\end{theorem}

\xhdr{Polynomial regret in (very) high dimension.}
In view of the $\sqrt{t}$ lower bound from Theorems~\ref{thm:main-experts}, we are interested in matching upper bounds. \citet{Anupam-experts07} observed that such bounds hold for every metric space $(X,\mD)$ of finite covering dimension: namely, the \FFproblem on $(X,\mD)$ is $\sqrt{t}$-tractable. (Their algorithm is a version of algorithm \NaiveAlg described in Section~\ref{sec:intro}.) Therefore it is natural to ask whether there exist metric spaces of \emph{infinite} covering dimension with polynomial regret.

We settle this question by proving a characterization with nearly matching upper and lower bounds in terms of a novel dimensionality notion tailored to the experts problem. We define the \emph{log-covering dimension} of $(X,\mD)$ as the smallest number $d\geq 0$ such that $X$ can be covered by
    $O\left(2^{r^{-d}} \right)$
sets of diameter $r$ for all $r>0$.
More formally:
\begin{align}\label{eq:LCD}
    \LCD(X) = \limsup_{r \to 0}\, \frac{\log\log N_r(X)}{\log (1/r)}.
\end{align}
where $N_r(X)$ is the minimal size (cardinality) of a $r$-covering of $X$, i.e. the smallest number of sets of diameter at most $r$ sufficient to cover $X$. Note that the number of sets allowed by this definition is exponentially larger than the one allowed by the covering dimension.

To give an example of a metric space with a non-trivial log-covering dimension, let us consider a \emph{uniform tree} -- a rooted tree in which all nodes at the same level have the same number of children. An \emph{\eps-uniform tree metric} is a metric on the ends of an infinitely deep uniform tree, in which the distance between two ends is $\eps^{-i}$, where $i$ is the level of their least common ancestor. It is easy to see that an \eps-uniform tree metric such that the branching factor at each level $i$ is
    $ \exp(\eps^{-id} (2^d - 1))$
has log-covering dimension $d$.

For another example, let $\mathcal{P}_X$ denote the set of all probability measures over $X=[0,1]^d$. Consider $\mathcal{P}_X$ as a metric space $(\mathcal{P}_X,W_1)$ under the Wasserstein $W_1$ metric, a.k.a. the Earthmover distance:
\begin{align*}
    W_1(\nu,\nu') = \inf \E\left[ \|Y-Y'\|_2 \right],
\end{align*}
where the infimum is taken over all joint distributions $(Y,Y')$ on $X\times X$
with marginals $\nu$ and $\nu'$ respectively (for any two
$\nu,\nu'\in \mathcal{P}_X$).
\footnote{\label{fn:earthmover}
The Wasserstein $W_1$ metric is one of the standard ways to define a distance on probability measures. In particular, it is widely used in Computer Science literature to compare discrete distributions, e.g. in the context of image retrieval \citep{earthmover-00}.}
We show that the log-covering dimension of this metric space is equal to the covering dimension of $(X,\mD)$. In fact, this example extends to any metric space $X$ of finite diameter and covering dimension $d$; see Appendix~\ref{app:earthmover} for the details.

\begin{theorem}\label{thm:intro-LCD}
Let $(X,\mD)$ be a metric space of log-covering dimension $d$. Then the \FFproblem is
 $(t^\gamma)$-tractable for any $\gamma> \tfrac{d+1}{d+2}$.
\end{theorem}

The algorithm in Theorem~\ref{thm:intro-LCD} is a version of \NaiveAlg. The same algorithm enjoys a better regret bound if each function $f\in \mathtt{support}(\mathbb{P})$ is itself a Lipschitz function on $(X,\mD)$. We term this special case the \emph{\ULproblem}. The analysis is much more sophisticated, using a chaining technique in empirical process theory. While our analysis is self-contained, background on chaining can be found in \citet{Talagrand-book05}.


\begin{theorem}\label{thm:intro-LCD-uniform}
Let $(X,\mD)$ be a metric space of log-covering dimension $d$. Then the \ULproblem is
 $(t^\gamma)$-tractable for any $\gamma> \tfrac{d-1}{d}$.
\end{theorem}

The proofs of these theorems can be found in Section~\ref{sec:FFproblem-LCD} and Section~\ref{sec:FFproblem-uniform}, respectively.

\xhdr{Per-metric optimal regret bounds.}
We find that the log-covering dimension is not the right notion to characterize optimal regret for arbitrary metric spaces. Instead, we define the \emph{max-min-log-covering dimension} ($\MaxMinLCD$): essentially, we take the definition of $\MaxMinCOV$ and replace covering dimension with log-covering dimension. \begin{align}\label{eq:MaxMinLCD}
\MaxMinLCD(X) = \textstyle{\sup_{Y\subset X}} \;
    \inf\{ \,\LCD(Z):\; \text{open non-empty $Z\subset Y$} \}.
\end{align}
\noindent Note that in general $\MaxMinLCD(X) \leq \LCD(X)$. Equality holds for ``homogeneous" metric spaces such as \eps-uniform tree metrics.
We derive the regret characterization in terms $\MaxMinLCD$; the characterization is tight for the \ULproblem.

\begin{theorem}\label{thm:intro-MaxMinLCD}
Let $(X,\mD)$ be an uncountable metric space and $d = \MaxMinLCD\geq 0$. Then:
\begin{OneLiners}
\item[(a)] the \FFproblem is $(t^\gamma)$-tractable for any $\gamma> \tfrac{d+1}{d+2}$,

\item[(b)] the \ULproblem is $(t^\gamma)$-tractable for any
    $\gamma> \max(\tfrac{d-1}{d}, \tfrac12)$,

\item[(c)] the \ULproblem is not $(t^\gamma)$-tractable for any $\gamma < \max(\tfrac{d-1}{d}, \tfrac12)$.
\end{OneLiners}
\end{theorem}

The algorithms in parts (a) and (b) use a generalization of the transfinite decomposition from the bandit per-metric optimal algorithm (Theorem~\ref{thm:intro.pmo}). The lower bound in part (c) builds on the lower-bounding technique for the $\sqrt{t}$ lower bound on uncountable metric spaces. The proof can be found in Section~\ref{sec:FFproblem-characterization}.

Our results for Lipschitz experts amount to a nearly complete characterization of per-metric optimal regret bounds, analogous to that in Table~\ref{tab:PMO-results} on page~\pageref{tab:PMO-results}.
This characterization is summarized in the table below.
(The characterization falls short of being complete because the
upper and lower bounds for finite $\MaxMinLCD = d \in [0,\infty)$
do not match.)

\begin{table}[h]
\label{tab:experts-results}
\caption{Per-metric optimal bounds for Lipschitz experts}
%\tbl{Per-metric optimal bounds for Lipschitz experts\label{tab:experts-results}}{%
\begin{tabular}{l|l|l}
If the completion of $(X,\mD)$ is ...  & then regret can be ...    & but not ... \\ \hline\\
compact and countable    & $O(1)$      & ~~--- \\
compact and uncountable  & & \\
~~~~~~~~~~~~ finite covering dimension
    & $\tilde{O}\left( \sqrt{t} \,\right)$
    & $o(\sqrt{t})$  \\
~~~~~~~~~~~~
$\MaxMinLCD=d\in [0,\infty)$
    & $\tilde{O}\left( t^\gamma \right)$, $\gamma >\tfrac{d+1}{d+2}$
    & $o\left( t^\gamma \right)$, $\gamma=\tfrac12$ or $\gamma <\tfrac{d-1}{d}$  \\
~~~~~~~~~~~~
$\MaxMinLCD=\infty$   & $o(t)$  & $O\left( t^\gamma \right)$, $\gamma<1$ \\
non-compact           & $O(t)$  & $o(t)$
\end{tabular}
\end{table}


\newcommand{\DpthOracle}{{\mathtt{Length}}}
\newcommand{\DCovOracle}{{\mbox{$\mD$-$\mathtt{Cov}$}}}

